Blueprint First, Model Second: A Framework for Deterministic LLM Workflow

While powerful, the inherent non-determinism of large language model (LLM) agents limits their application in structured operational environments where procedural fidelity and predictable execution are strict requirements. This limitation stems from current architectures that conflate probabilistic, high-level planning with low-level action execution within a single generative process. To address this, we introduce the \textsc{Source Code Agent} framework, a new paradigm built on the ``Blueprint First, Model Second'' philosophy that decouples workflow logic from the generative model. An expert-defined operational procedure is first codified into a source code-based Execution Blueprint, which is then executed by a deterministic engine. The LLM is strategically invoked as a specialized tool to handle bounded, complex sub-tasks within the workflow, but never to decide the workflow's path. We evaluate on the TravelPlanner benchmark for constraint-aware travel planning. The \textsc{Source Code Agent} achieves a 35.56\% final pass rate, a 97.6\% improvement over the state-of-the-art ATLAS baseline (18.00\%) on the same Claude-Sonnet-4 backbone. Critically, it reduces constraint violations by 96.0\% (11 vs 275) while improving execution efficiency by 27.1\% (10.2$\pm$0.7 steps vs 14.0). Two production incident-diagnosis deployments and additional results on ScienceWorld and ALFWorld confirm that the architecture transfers beyond travel planning to procedurally well-defined, constraint-intensive workflows. Our work enables the verifiable and reliable deployment of autonomous agents in applications governed by strict procedural logic.

==> chapter/checklist.tex <==
\section{Reproducibility Checklist}
\label{sec:checklist}

Unless specified otherwise, please answer ``yes'' to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled ``Reproducibility Checklist'' at the end of the technical appendix.



This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)
\end{itemize}

Does this paper make theoretical contributions? (no)

Does this paper rely on one or more datasets? (yes)

If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes)
    \item All novel datasets introduced in this paper are included in a data appendix. (yes)
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes)
\end{itemize}


Does this paper include computational experiments? (yes)

If yes, please complete the list below.
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (yes).
    \item All source code required for conducting and analyzing the experiments is included icode apdix. (yes)
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
    \item This paper states the number of algorithm runs used to compute each reported result. (yes)
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes)
\end{itemize}

==> chapter/preliminary.tex <==
\section{Background and Related Work}
\label{sec:preliminary}

Our work is situated at the intersection of two pivotal areas in modern AI research: enhancing the reasoning capabilities of LLMs and constructing sophisticated agentic systems. In this section, we review the foundational literature in both domains, analyzing their contributions and identifying the architectural gaps that motivate our proposed framework.

\subsubsection{Chain-of-Thought (CoT) }
The ability to perform complex, multi-step reasoning is a cornerstone of intelligence. For LLMs, a significant breakthrough in this area was the introduction of CoT prompting~\cite{wei2022chain}. Instead of directly outputting an answer, CoT encourages the model to generate a series of intermediate, step-by-step reasoning traces that lead to the final conclusion. This process was shown to dramatically improve performance on tasks requiring arithmetic~\cite{arithmetic2024cot}, commonsense~\cite{commonsense}, and symbolic reasoning~\cite{symbolic} by allowing the model to decompose complex problems into more manageable sub-problems.

Building on this foundation, a rich body of work has emerged to refine and enhance structured reasoning. For example, Tree of Thoughts (ToT)~\cite{yao2023tree} generalizes CoT by enabling the model to explore multiple reasoning paths concurrently in a tree structure, using self-evaluation to select the most promising path. Other approaches, such as Graph of Thoughts (GoT)~\cite{besta2024graph}, further extend this by modeling reasoning processes as arbitrary graphs, allowing for more complex thought aggregation and transformation.

A critical challenge in this domain, however, is the quality and reliability of the generated reasoning steps. Since the ``thoughts" are produced by the probabilistic LLM itself, they can be prone to factual errors, logical fallacies, and hallucinations. To mitigate this, multiple research directions have been explored. One notable direction involves improving the supervision data for fine-tuning by leveraging the determinism of program execution to generate high-quality CoT datasets~\cite{jung2025code}. By executing code, which has verifiable outcomes, researchers can extract step-by-step traces and translate them into natural language reasoning paths. Another approach, SymbCoT~\cite{xu2024faithful}, aims to enhance the reasoning process directly by integrating symbolic representations and logical rules into CoT prompts, thereby grounding the model's reasoning in a more formal structure.

\textbf{Limitations and Our Position:} While these advancements have significantly improved the internal reasoning quality of LLMs, they do not address the core challenge of external execution determinism. The primary goal of CoT and its variants is to elicit a more robust thought process, but the process itself remains a generative and fundamentally non-deterministic act. Even when trained on program-verified data, the model is not constrained to follow a specific execution path at runtime. This leaves a critical gap for applications where the sequence of external actions (e.g., tool calls, API requests) must be predictable and guaranteed, not merely the internal rationale.


\subsubsection{Agentic Systems}
The paradigm of AI agents has moved beyond single-function models to become complex, autonomous systems that can perceive their environment, plan, and act to achieve goals~\cite{guo2024large}. Modern agentic systems typically use an LLM as a central controller or ``brain" to orchestrate a loop of reasoning and action~\cite{wang2024survey}. A foundational architecture in this space is ReAct (Reason and Act)~\cite{yao2022react}, which interleaves reasoning traces (similar to CoT) with actions, such as calling external tools. This enables the agent to dynamically plan its next steps based on observations from the environment. Alternatively, other influential architectures emphasize more structured, upfront planning. For example, Wang et al.~\cite{wang2023plan} proposed a ``plan-and-solve" paradigm, where the agent first devises a comprehensive plan to decompose the entire task into smaller sub-tasks and then proceeds to execute them according to that established plan.

The power of these agents is greatly amplified by their ability to use external tools~\cite{masterman2024landscape}. Frameworks like Toolformer~\cite{schick2023toolformer} and Gorilla~\cite{patil2024gorilla} have demonstrated how LLMs can be trained to master a vast number of APIs, allowing them to search for information, execute code, or interact with databases. This has led to the development of sophisticated, multi-agent, or compound systems that integrate multiple specialized components and tools to solve complex, real-world problems~\cite{yang2024swe, hong2023metagpt}. To manage the complexity, mechanisms for self-reflection and refinement have also been proposed, where an agent can critique its own work and iteratively improve its plan or output, as seen in systems like Reflexion~\cite{shinn2023reflexion}.

\textbf{Limitations and Our Position:}  Despite their impressive capabilities, the autonomy of current agentic systems is a double-edged sword. Their operational flow is predominantly guided by the LLM controller's probabilistic decisions. When faced with a task, the agent's choice of which tool to use, what parameters to provide, and how to interpret the results is generated "on the fly." As illustrated by our troubleshooting example in the introduction, this can lead to inefficient, unpredictable, or even erroneous execution paths. While this flexibility is desirable for exploration, it is a liability in structured, high-stakes environments. The engineering effort required to constrain these agents and ensure reliable behavior for specific workflows is substantial and often involves brittle, ad hoc prompt engineering.

In summary, the related work in both CoT and agentic systems has pushed the boundaries of what AI can achieve. However, their design prioritizes generative flexibility over procedural fidelity. There is a clear need for a new architectural pattern that can harness the specialized intelligence of LLMs while enforcing a deterministic and verifiable execution workflow. EBF is designed to fill this precise gap by separating the rigid, predefined process flow from the flexible, model-driven execution of individual tasks.




